Towards Online Monitoring and Data-driven Control: A Study of Segmentation Algorithms for Laser Powder Bed Fusion Processes

An increasing number of laser powder bed fusion machines use off-axis infrared cameras to improve online monitoring and data-driven control capabilities. However, there is still a severe lack of algorithmic solutions to properly process the infrared images from these cameras that has led to several key limitations: a lack of online monitoring capabilities for the laser tracks, insufficient pre-processing of the infrared images for data-driven methods, and large memory requirements for storing the infrared images. To address these limitations, we study over 30 segmentation algorithms that segment each infrared image into a foreground and background. By evaluating each algorithm based on its segmentation accuracy, computational speed, and spatter detection characteristics, we identify promising algorithmic solutions. The identified algorithms can be readily applied to the laser powder bed fusion machines to address each of the above limitations and thus, significantly improve process control.

==> image_matrix_2.tex <==
\begin{figure*}[tb]
    \centering % <-- added
    
\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth308.png}
\subcaption[]{Segmentation ground truth. Black marks the buffer zone, red the foreground, and yellow the background.}   
\end{subfigure}

\medskip

% \begin{subfigure}{\textwidth}
%   \includegraphics[width=0.12\linewidth]{imgs/MOG302.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG303.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG304.png}
%       \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG305.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG306.png}
%       \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG307.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG308.png}
% \subcaption[]{MOG}
% \end{subfigure}

% \medskip



\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG2307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG2308.png}
\subcaption[]{MOG}
\end{subfigure}

\medskip


\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG308.png}
\subcaption[]{GMG}
\end{subfigure}

\medskip

% \begin{subfigure}{\textwidth}
%   \includegraphics[width=0.12\linewidth]{imgs/KNN302.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN303.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN304.png}
%       \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN305.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN306.png}
%       \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN307.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN308.png}
% \subcaption[]{KNN}
% \end{subfigure}

% \medskip

\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu308.png}
\subcaption[]{Otsu's method}
\end{subfigure}

\caption{Segmentation results of different algorithms with mediocre or poor performance for an exemplary sequence of infrared images. The images are cropped to the area of the first cross-section.}

\label{fig:segment_poor_results}

\end{figure*}


==> image_matrix_backup.tex <==
\begin{figure*}[p]
    \centering % <-- added
    
\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth]{imgs/No method302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/No method303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/No method304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/No method305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/No method306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/No method307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/No method308.png}
\subcaption[]{Cropped raw infrared images from the SLS build (images from the same layer as Figure \ref{fig:mask_sub1})}
\end{subfigure}
\medskip

\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth308.png}
\subcaption[]{Segmentation ground truth. Black marks the buffer zone, red the foreground, and yellow the background.}   
\end{subfigure}
\medskip

\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction308.png}
\subcaption[]{FD + Thresh($\lambda$)}   
\end{subfigure}
\medskip

\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth]{imgs/FD_GSOC302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_GSOC303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_GSOC304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_GSOC305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_GSOC306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_GSOC307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_GSOC308.png}
\subcaption[]{FD + GSOC}
\end{subfigure}

\medskip

\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction dynamic Yen302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction dynamic Yen303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction dynamic Yen304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction dynamic Yen305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction dynamic Yen306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction dynamic Yen307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/Subtraction dynamic Yen308.png}
\subcaption[]{FD + Yen}   
\end{subfigure}
\medskip

\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth]{imgs/FD_CNT302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_CNT303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_CNT304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_CNT305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_CNT306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_CNT307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/FD_CNT308.png}
\subcaption[]{FD + CNT}
\end{subfigure}

\medskip

\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth]{imgs/trivial HAZ thresh302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/trivial HAZ thresh303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/trivial HAZ thresh304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/trivial HAZ thresh305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/trivial HAZ thresh306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/trivial HAZ thresh307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/trivial HAZ thresh308.png}
\subcaption[]{Baseline}
\end{subfigure}

\caption{Segmentation results of the top-performing algorithms for an exemplary sequence of infrared images. The images are cropped to the area of the first cross-section.}
\label{fig:segment_results}

\end{figure*}


==> image_matrix_backup_2.tex <==
\begin{figure*}[tb]
    \centering % <-- added
    
\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth]{imgs/ground_truth308.png}
\subcaption[]{Segmentation ground truth. Black marks the buffer zone, red the foreground, and yellow the background.}   
\end{subfigure}

\medskip

% \begin{subfigure}{\textwidth}
%   \includegraphics[width=0.12\linewidth]{imgs/MOG302.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG303.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG304.png}
%       \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG305.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG306.png}
%       \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG307.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/MOG308.png}
% \subcaption[]{MOG}
% \end{subfigure}

% \medskip



\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG2307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/MOG2308.png}
\subcaption[]{MOG}
\end{subfigure}

\medskip


\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/GMG308.png}
\subcaption[]{GMG}
\end{subfigure}

\medskip

% \begin{subfigure}{\textwidth}
%   \includegraphics[width=0.12\linewidth]{imgs/KNN302.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN303.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN304.png}
%       \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN305.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN306.png}
%       \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN307.png}
%     \hfil % <-- added
%   \includegraphics[width=0.12\linewidth]{imgs/KNN308.png}
% \subcaption[]{KNN}
% \end{subfigure}

% \medskip

\begin{subfigure}{\textwidth}
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu302.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu303.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu304.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu305.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu306.png}
      \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu307.png}
    \hfil % <-- added
  \includegraphics[width=0.115\linewidth, frame]{imgs/Otsu308.png}
\subcaption[]{Otsu's method}
\end{subfigure}

\caption{Segmentation results of different algorithms with mediocre or poor performance for an exemplary sequence of infrared images. The images are cropped to the area of the first cross-section.}

\label{fig:segment_poor_results}

\end{figure*}


==> table_f1_precision_recall.tex <==
\begin{table}
    \centering
    \caption{Performance of tested algorithms.}
    \captionsetup{justification=centering}
    \begin{tabular}{llllr}
        \toprule
        Algorithms & Parameters & Precision & Recall & F1-score \\
        \midrule
        \multirow{2}{*}{FD}   & calibrated     & 0.98       & 0.92        & 0.95 \\
        {}                                  & default        & 0.83       & 0.95        & 0.89 \\
        \addlinespace[8pt]

        \multirow{2}{*}{MOG}                & calibrated    & 0.59       & 0.79         & 0.68 \\
        {}                                  & default       & 0.27        & 0.89        & 0.42 \\
        \addlinespace[8pt]
        
        \multirow{2}{*}{MOG2}               & calibrated    & 0.74       & 0.74         & 0.74\\
        {}                                  & default       & 0.16       & 0.98         & 0.28 \\
        \addlinespace[8pt]
        
        \multirow{2}{*}{KNN}                & calibrated    & 0.56       & 0.78         & 0.67 \\
        {}                                  & default       & 0.13       & 0.97         & 0.23 \\
        \addlinespace[8pt]
        
        \multirow{2}{*}{GMG}                & calibrated    & 0.85       & 0.67         & 0.75\\
        {}                                  & default       & 0.48        & 0.89         & 0.62 \\
        \addlinespace[8pt]
        
        \multirow{2}{*}{CNT}                & calibrated    & 0.56       & 0.83         & 0.67\\
        {}                                  & default       & 0.18       & 0.92         & 0.30 \\
        \addlinespace[8pt]

        \multirow{2}{*}{SubMax}    & calibrated    & 0.70       & 0.62         & 0.66 \\
        {}                                  & default       & 1.00       & 0.02         & 0.04 \\
        \addlinespace[8pt]
        
        \multirow{2}{*}{GSOC}               & calibrated    & 0.91       & 0.37         & 0.52\\
        {}                                  & default       & 0.09       & 1.00         & 0.16 \\
        \addlinespace[8pt]

        \multirow{2}{*}{AdaptMean}      & calibrated    & 0.00       & 1.00         & 0.00 \\
        {}                                  & default       & 0.00       & 0.83         & 0.00 \\
        \addlinespace[8pt]
        
        \multirow{2}{*}{AdaptGauss}  & calibrated    & 0.00       & 1.00         & 0.00 \\
        {}                                  & default       & 0.00       & 0.76         & 0.00 \\
        \addlinespace[8pt]
        
        \multirow{2}{*}{Sauvola}            & calibrated    & 0.00       & 1.00         & 0.00 \\
        {}                                  & default       & 0.00       & 1.00         & 0.00 \\
        \addlinespace[8pt]
        
        Otsu                                & \multicolumn{1}{c}{--}      & 0.01       & 0.95         & 0.03 \\
        \addlinespace[8pt]
        
        Li                                  & \multicolumn{1}{c}{--}       & 0.00       & 1.00      &   0.00\\
        \addlinespace[8pt]
        
        Yen                                 & \multicolumn{1}{c}{--}       & 0.00       & 1.00      & 0.00\\
        \addlinespace[8pt]
        
        isodata                             & \multicolumn{1}{c}{--}     & 0.00       & 1.00        & 0.00\\
        \addlinespace[8pt]

        Triangle                            & \multicolumn{1}{c}{--}     & 0.04       &1.00         & 0.09 \\
        \addlinespace[8pt]

        
        
        \bottomrule
    \end{tabular}
    \label{table:F1_score}
\end{table}

==> table_total_results_long_table.tex <==
\begin{longtable*}
    \centering
    \caption{Performance summary of all algorithms (Part 1).}
    \captionsetup{justification=centering}
    \begin{tabular}{llccccc}
        \toprule
        \multicolumn{2}{c}{\multirow{2}{*}[-1em]{Algorithms}} & \multicolumn{3}{c}{Segmentation accuracy} & Computation time & {Spatter robust?} \\
        \addlinespace[10pt]
        \cmidrule(lr){3-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}\\
        {} & {} & Precision & Recall & F\textsubscript{1}-score  & [\si{ms}] \\
        \midrule
        
\multirow{2}{*}{Thresh($\lambda$)} & default        & 0.09 & 0.98 & 0.17 & \multirow{2}{*}{0.21} & \multirow{2}{*}{No} \\
&calibrated		                 & 0.61 & 0.63 & 0.62 &  & \\
        \addlinespace[5pt]         
 
FD & \multicolumn{1}{c}{--}		                         & 0.00 & 1.00 & 0.00 & 0.29 & No\\
        \addlinespace[5pt]         

\multirow{2}{*}{MOG} & default                      & 0.21 & 0.90 & 0.35 & \multirow{2}{*}{5.17} & \multirow{2}{*}{Yes}\\
&calibrated                                      & 0.46 & 0.81 & 0.58 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+MOG} & default             & 0.54 & 0.68 & 0.60 & \multirow{2}{*}{5.33} & \multirow{2}{*}{No}\\
&calibrated                                    & 0.66 & 0.67 & 0.67 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{MOG2} & default                & 0.10 & 0.96 & 0.17 & \multirow{2}{*}{2.31} & \multirow{2}{*}{Yes}\\
&calibrated                                     & 0.17 & 0.87 & 0.29 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+MOG2} & default            & 0.21 & 0.79 & 0.33 & \multirow{2}{*}{3.32} & \multirow{2}{*}{No}\\
&calibrated                                   & 0.22 & 0.93 & 0.35 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{KNN} & default                   & 0.06 & 0.97 & 0.10 & \multirow{2}{*}{2.59} & \multirow{2}{*}{Yes}\\
&calibrated                                      & 0.08 & 0.96 & 0.14 & & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+KNN} & default                             & 0.12 & 0.81 & 0.21 & \multirow{2}{*}{5.19} & \multirow{2}{*}{No}\\
&calibrated                                    & 0.13 & 0.95 & 0.22 & & \\
        \addlinespace[5pt]         

\multirow{2}{*}{GMG} & default                               & 0.17 & 0.89 & 0.29 & \multirow{2}{*}{8.44} & \multirow{2}{*}{No}\\
&calibrated                                      & 0.17 & 0.89 & 0.29 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+GMG} & default                             & 0.23 & 0.80 & 0.36 & \multirow{2}{*}{9.39} & \multirow{2}{*}{No}\\
&calibrated                                    & 0.24 & 0.95 & 0.38 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{CNT} & default                               & 0.02 & 0.94 & 0.04 & \multirow{2}{*}{0.74} & \multirow{2}{*}{Yes}\\
&calibrated                                      & 0.42 & 0.81 & 0.56 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+CNT} & default                             & 0.02 & 0.73 & 0.03 & \multirow{2}{*}{1.67} & No\\
&calibrated                                    & 0.67 & 0.73 & 0.70 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+Thresh($\lambda$)} & default    & 0.85 & 0.93 & 0.88 & \multirow{2}{*}{0.47} & No\\
&calibrated                              & 0.95 & 0.90 & 0.93 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{SubMax($\delta$)} & default                    & 0.00 & 0.07 & 0.00 & \multirow{2}{*}{0.96} & No\\
&calibrated                           & 0.00 & 0.65 & 0.01 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{GSOC} & default                              & 0.07 & 1.00 & 0.13 & \multirow{2}{*}{267.37} & \multirow{2}{*}{Yes}\\
&calibrated                                     & 0.66 & 0.55 & 0.60 & & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+GSOC} & default          & 0.26 & 0.87 & 0.41 & \multirow{2}{*}{296.03} & \multirow{2}{*}{No}\\
&calibrated                                   & 0.91 & 0.78 & 0.84 &  & \\

        \addlinespace[5pt]         

\multirow{2}{*}{LSBP} & default                              & 0.16 & 0.73 & 0.26 & \multirow{2}{*}{16.83} & \multirow{2}{*}{No}\\
&calibrated                                     & 0.18 & 0.68 & 0.29 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+LSBP} & default                            & 0.01 & 0.59 & 0.01 & \multirow{2}{*}{16.00} & \multirow{2}{*}{No}\\
&calibrated                                   & 0.01 & 0.56 & 0.01 &  & \\


\multirow{2}{*}{AdaptMean} & default                      & 0.00 & 0.85 & 0.00 & \multirow{2}{*}{1.21} & \multirow{2}{*}{No}\\
&calibrated                             & 0.00 & 1.00 & 0.00 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{AdaptGauss} & default                  & 0.00 & 0.77 & 0.00 & \multirow{2}{*}{15.77} & \multirow{2}{*}{No}\\
&calibrated                         & 0.00 & 1.00 & 0.00 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+AdaptMean} & default  & 0.00 & 0.71 & 0.00 & \multirow{2}{*}{1.40} & \multirow{2}{*}{No}\\
&calibrated			         & 0.00 & 1.00 & 0.00 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+AdaptGauss} & default & 0.00 & 0.60 & 0.00 & \multirow{2}{*}{1.66} & \multirow{2}{*}{No}\\
&calibrated				 & 0.00 & 1.00 & 0.00 &  & \\
        \addlinespace[5pt]         

Otsu                       & \multicolumn{1}{c}{--}              & 0.00 & 0.96 & 0.01 & 0.72 & No\\
        \addlinespace[5pt]         

Li                         & \multicolumn{1}{c}{--}              & 0.00 & 1.00 & 0.00 & 9.21 & No\\
        \addlinespace[5pt]         

\multirow{2}{*}{Sauvola} & default                           & 0.00 & 0.91 & 0.00 & \multirow{2}{*}{8.36} & \multirow{2}{*}{No}\\
&calibrated                                  & 0.00 & 1.00 & 0.00 &  & \\
        \addlinespace[5pt]         

\multirow{2}{*}{FD+Sauvola} & default                         & 0.35 & 0.79 & 0.48 & \multirow{2}{*}{23.74} & \multirow{2}{*}{No}\\
&calibrated                                & 0.39 & 0.90 & 0.54 &  & \\
        \addlinespace[5pt]         

Triangle                   & \multicolumn{1}{c}{--}              & 0.01 & 1.00 & 0.02 & 0.69 & No\\
        \addlinespace[5pt]         

Yen & \multicolumn{1}{c}{--}  		 & 0.01 & 0.91 & 0.02 & 1.10 & No\\
        \addlinespace[5pt]         

isodata & \multicolumn{1}{c}{--}         & 0.00 & 1.00 & 0.00 & 1.12 & No\\
        \addlinespace[5pt]         

FD+Otsu     & \multicolumn{1}{c}{--}              & 0.62 & 0.59 & 0.60 & 1.15 & No\\
        \addlinespace[5pt]         

FD+Li       & \multicolumn{1}{c}{--}              & 0.36 & 0.94 & 0.52 & 7.02 & No\\
        \addlinespace[5pt]         

FD+Triangle & \multicolumn{1}{c}{--}              & 0.44 & 0.95 & 0.60 & 1.09 & No\\
        \addlinespace[5pt]         

FD+Yen      & \multicolumn{1}{c}{--}              & 0.73 & 0.84 & 0.78 & 1.51 & No\\
        \addlinespace[5pt]         

FD+isodata  & \multicolumn{1}{c}{--}              & 0.62 & 0.59 & 0.61 & 1.50 & No\\

        \bottomrule
    \end{tabular}
    \label{table:all_results1}
\end{longtable*}
